007: Democratically Finding The Cause of Packet Drops

Network failures continue to plague datacenter operators as their symptoms may not have direct correlation with where or why they occur. We introduce 007, a lightweight, always-on diagnosis application that can find problematic links and also pinpoint problems for each TCP connection. 007 is completely contained within the end host. During its two month deployment in a tier-1 datacenter, it detected every problem found by previously deployed monitoring tools while also finding the sources of other problems previously undetected.

==> eval-tr.tex <==
\section{Evaluations: Simulations}
\label{sec:sim}
\vspace{1mm}

We start by evaluating in simulations where we know the ground
truth. In these simulations, \Sys first finds connections whose drops
were due to noise and marks them as ``noise drops''. It then finds the
link most likely responsible for packet drops on the remaining set of
connections~(``failure drops''). A noisy drop is defined as one where
the link responsible for the drop only dropped a single packet. We
found that \Sys never marked a connection into the noisy category
incorrectly. We therefore focus on the accuracy for connections that
\Sys puts into the failure drop class.


\noindent{\bf Performance metrics.} Our primary measure for
performance for \Sys is \emph{detection accuracy}, which is defined as
the likelihood of being able to correctly identify the cause of a
failed connection~(e.g., pinpoint the correct link that failed). For
simplicity, we refer to this only as \emph{accuracy} in this
section. For evaluating Algorithm~\ref{alg:vigil}, we use the
alternative performance metrics of {\em recall} and {\em
  precision}. Recall is a measure of reliability and shows how many of
the failures \Sys can accurately detect~(false negatives). For
example, if there are 100 failed links and \Sys detects 90 of them,
its recall is $90\%$. Precision is a measure of accuracy and shows to
what extent the \Sys's results can be trusted~(false positives). For
example, if \Sys flags 100 links as bad, but only 90 of those links
actually failed, its precision is $90\%$.


\noindent{\bf Simulation setup.} We use a flow level simulator
implemented in MATLAB. Our simulated topology consists of $4160$
links, $2$ pods, $20$ ToRs per pod. Each host in the simulator
establishes $2$ connections per second to a random ToR in the network
outside of its rack. The simulator has two types of links. For {\em
  good links} that are operating without failure, packets are dropped
at a very low rate chosen uniformly from $(0,10^{-6})$ to simulate
noise. On the other hand, {\em failed links} have a much higher drop
rate to simulate failures. By default, drop rates on failed links are
set to vary uniformly from $0.01$\% to $0.1$\%, though to study the
impact of drop rates, we do allow this rate to vary as an input
parameter. The number of good and failed links is also a tunable
simulation parameter. Every $30$ seconds of simulation time, we send
up to $100$ packets per connection, and drop packets based on the
rates above as they traverse links along the connection. The simulator
records all connections with at least one packet drop, for each such
connection, the link with the most drops.

As a basis for comparison, we compare \Sys against the optimal
solution described in in \S\ref{sec:optimal}. We refer to the optimal
solution as ``Integer Optimization'' in the figures, and
``optimization'' in the text when comparing with \Sys.

%%% REMOVE AS CONFUSING %%%%
%In order to allow a fair comparison to the optimization algorithm
%(\S~\ref{sec:optimal}), we also record the path of $15\%$ of good
%connections \textit{only} as input for the optimization (we do not use
%these values to calculating our votes).


\subsection{In the optimal case}
\vspace{1mm}

%\noindent{\textbf{Finding the cause of packet drops.}} 

%The simulation setup described earlier does not satisfy the bounds in
%Theorem~\ref{T:vigilWorks}. This is to demonstrate that these bounds
%while sufficient, are not necessary for the good performance of
%\Sys. 

In our first experiment, we use simulation settings where the bounds
in Theorem~\ref{T:vigilWorks} do hold. Recall that these bounds are
sufficient conditions for \Sys's accuracy. The first experiment aims to
validate that \Sys can trivially achieve high levels of accuracy as
expected. Given the simulation setup above, we set the drop rates on
the failed links to be between $(0.05\%,1\%)$. At drop rates below
$0.05\%$, the theorem bounds will no longer hold.

%Recall that if the
%bounds hold, \Sys is thereotically supposed to perform with high
%levels of accuracy.

\noindent {\bf Accuracy.} Figure~\ref{fig:theorem2} shows that \Sys
has an average accuracy that is higher than $96\%$ in almost all
cases. Furthermore, due to its robustness to noise, it also
outperforms the optimization algorithm~(\S~\ref{sec:optimal}) in most
cases.

%\noindent{\textbf{In the case of Algorithm~\ref{alg:vigil}.}}

\noindent {\bf Recall and precision.} Figure~\ref{fig:reasonable}
shows that even with low packet drop rates on the failed links, \Sys
detects the failed links with high recall and precision. This confirms
that when the conditions in Theorem~\ref{T:vigilWorks} hold, \Sys can
be trusted to find the right set of links.

In the rest of this section, we proceed to evaluate \Sys's performance
when the conditions in Theorem~\ref{T:vigilWorks} {\em do not} hold
(i.e. packet drop rates below $0.05\%$). This illustrates that while
sufficient, these conditions are not necessary for the good
performance of \Sys.


\begin{figure}[tb]
	\centering
	\includesvg{Theorem2}
	\caption{When Theorem 2 holds.}
		\label{fig:theorem2}
\end{figure}


\begin{figure}[tb]
	\centering
	\includesvg{reasonable-tr}
	\caption{ Testing Algorithm~\ref{alg:vigil} when Theorem 2 holds.}
		\label{fig:reasonable}
\end{figure}



\subsection{Varying Drop Rates}
\vspace{1mm}
\label{sec:Drops}

Our next experiment aims to push the boundaries of
Theorem~\ref{T:vigilWorks} by varying the ``failed'' links drop rates well
below the conservative bounds of Theorem~\ref{T:vigilWorks}.

%%Although we analytically evaluated the drop rates that \Sys can
%detect~(see~\S\ref{sec:vote}), our calculations are based on
%conservative bounds and shows that for a single failure, links with
%packet drop rates as low as~$0.05\%$ can be detected.

\noindent{\textbf{Single Failure.}} Figure~\ref{fig:dropRate}a shows
simulation results for different drop rates on a single failed link in
the network. Our results show that for high drop rates, \Sys can find
the cause of packet drops on each connection with high accuracy. Even
as the drop rate decreases below the $0.05\%$ bound obtained from
Theorem~\ref{T:vigilWorks}, we observe that \Sys is still able to
maintain a high level of accuracy ($\ge 80\%$), on par with the
optimal solution.

%Indeed, for a drop rate of~$0.05\%$, \Sys's accuracy is
%$\ge 80\%$~($90\%$ for drop rates higher than $0.1\%$).

\noindent{\textbf{Multiple Failures.}} A noted shortcoming of past
work has been in identifying problematic links in the network where
the failed links have very different drop rates~\cite{alex}.  We test
\Sys's ability to find the cause of packet drops in the presence of
such failures. Figure~\ref{fig:dropRate}b illustrates this point for
different number of failed links under the default drop rate setting
described in the simulation setup. \Sys is almost always successful at
identifying the link responsible for a packet drop. In fact, it {\em
  surpasses} the optimization algorithm (albeit slightly) in
\S\ref{sec:optimal}. This is due to the optimization's susceptibility
to lone packet drops due to noise.


\begin{figure}[t]
	\centering
	\includesvg{dropRate}
	\caption{\Sys's accuracy for varying drop rates.}
		\label{fig:dropRate}
\end{figure}
\


\subsection{Impact of Noise}
	\label{sec:Noise}
\vspace{1mm}

\noindent{\textbf{Single Failure.}} We next vary the level of noise in
the network to see how well \Sys can attribute the cause of packet
drops in the presence of various degrees of noise. This is done by
changing the drop rate of the good links across different experimental
runs. Figure~\ref{fig:noise}a shows the accuracy results in the case
of a single link failure as the drop rate varies. Higher noise levels
could make it harder for \Sys to detect the link failure through
Algorithm~\ref{alg:vigil}. However, as shown in Figure~\ref{fig:noise}
they have little impact on its ability to find the cause of packet
drops on individual connections.

\noindent{\textbf{Multiple Failures.}} We repeat this experiment for
the case of $5$ failed links. Figure~\ref{fig:noise}b shows the
results. Again, \Sys shows little sensitivity to the increase in noise
when identifying the cause of per-connection packet drops. Note that
the large confidence intervals of the integer optimization problem
show its high sensitivity to noise.

%failures where we use $k=5$ as the number of
%failed links. 




\vspace{1mm}

\begin{figure}[hbt]
  \centering
\includegraphics[width=1\linewidth]{Figures/noise.pdf}
\caption{\Sys's accuracy for varying noise levels. Lone/sporadic drops are not 
of interest to a network provider/operator. \Sys can successfully ignore such drops and continue to 
perform well in the presence of high degrees of noise.}
		\label{fig:noise}
\end{figure}

%%For these results look into the file Sensitivity Analysis on my mac.




\subsection{Varying Number of Connections}
\label{sec:singleNumCon}
\vspace{1mm}

In previous experiments, all hosts
opened~$2$ connections per second. Here, we allow hosts to choose the
number of connections they create in each epoch uniformly at random
between $(10,60)$. Recall from Theorem~\ref{T:vigilWorks} that a
larger number of connections from each host helps \Sys improve its
accuracy. 

\noindent{\textbf{Single Failure.}}  Figure~\ref{fig:connections}a
validates this effect for the case of a single filed link. Our results show
that \Sys accurately identify the cause of packet drops
on connections with high probability. \Sys also significantly
outperform the optimization when the failed link has a low packet
drop rate. This is because the optimization has multiple optimal
points and is not sufficiently constrained.

%shows the result of varying the number of connections when there are
%multiple failed links. 

\noindent{\textbf{Multiple Failures.}} Figure~\ref{fig:connections}b
repeats the same experiment as above, but we vary the number of failed
links under the default drop rate settings.  The integer optimization
problem suffers from the lack of information to constrain the set of
results. It therefore has a huge variance (shown in terms of
confidence intervals). \Sys on the other hand maintains high
probability of detection (at low variance) no matter the number of
failed links.



\begin{figure}[hbt]
  \centering
\includegraphics[width=1\linewidth]{Figures/conn.pdf}
\caption{\Sys's accuracy for varying number of connections. Each host opens between $(10,60)$ connections. Where the number
is chosen unifromly at random.}
		\label{fig:connections}
\end{figure}




\subsection{Impact of Traffic Skews}
	\label{sec:singleSkew}
	\vspace{1mm}

\noindent{\textbf{Single Failure.}} We next demonstrate \Sys's ability
to detect the cause of connection packet drops even when traffic is
heavily skewed. We pick $10$ ToRs at random from the set of all ToRs
in the network ($25\%$ of the ToRs). To skew the traffic, 80\% of the
connections have destinations set to hosts under these $10$ ToRs, an
the remaining connections route to hosts randomly chosen in the
network. Figure~\ref{fig:trafficSkew}a shows that despite the traffic
skews, the optimization is much more heavily impacted by the skew than
\Sys. \Sys continues to detect the cause of packet drops with high
probability ($\ge 85\%$) for drop rates higher than $0.1\%$.

%Connections are biased to have
%hosts under these ToRs as destinations with probability $0.8$ and
%otherwise pick a ToR uniformly at random from the set of {\em all}
%ToRs in the network. This heavily skews the traffic to be biased
%towards these ToRs. 

\begin{figure}[hbt]
  \centering
\includegraphics[width=1\linewidth]{Figures/skew.pdf}
     \caption{\Sys's accuracy under heavily skewed traffic. The large confidence intervals of the optimization problem
  are a reflection of its sensitivity to noise.}
		\label{fig:trafficSkew}
\end{figure}





\noindent{\textbf{Multiple Failures.}} We repeated the above
experiment for multiple failures. Figure~\ref{fig:trafficSkew}b shows
that the optimization's accuracy suffers. It consistently shows a low
detection rate as its constraints are not sufficient in guiding the
optimizer to the right solution. On the other hand ,\Sys maintains a
detection rate of $\ge 98\%$ at all times.







\subsection{Detecting Bad Links}
\label{sec:singleAlg}
\vspace{1mm}
%%Single failure

In all our previous experiments, the focus has been on detection
accuracy from each connection's point of view. In our next experiment,
we evaluate \Sys's ability to detect bad links using the metrics of
recall and precision.

\noindent{\textbf{Single Failure.}} Figure~\ref{fig:alg1Single} shows
the results for finding the failed link in the network using
Algorithm~\ref{alg:vigil}. In the presence of a single failure, our
approach outperforms the optimization algorithm as it does not require
a fully specified set of equations in order to provide a best guess as
to which link is failed.

\noindent{\textbf{Multiple Failures.}}  In this scenario, the drop
rates on the failed links are heavily skewed. More specifically, at
least one failed link is assigned a drop rate in the range of
$(10\%,100\%)$ while all others have a drop rate in
$(0.01\%,0.1\%)$. This scenario is one where past approaches have
reported as potentially hard to detect~\cite{alex}.
Figure~\ref{fig:alg1Multiple} shows that \Sys can detect up to $7$
failures with recall/precision above $90\%$. However, its recall drops
as the number of failed links increase. This is due to the fact that
the increase in the number of failures drives up the votes of all
other links increasing the cutoff threshold and therefore increasing
the likelihood of false negatives. In fact if instead the top $k$
links had been selected \Sys's recall would have been close to
$100\%$~\cite{VigilProofs}. Further evaluations can be found
in~\cite{VigilProofs}.




\begin{figure}[hbt]
  \centering
	\includesvg[width=\linewidth]{alg1_single-tr}
     \caption{Algorithm~\ref{alg:vigil} with single failure. \Sys can accurately detect the cause of
     problems with recall/precision above $90\%$. However, its recall drops
as the number of failed links increase. }
     \label{fig:alg1Single}
     \vspace{2mm}
\end{figure}

\begin{figure}[hbt]
  \centering
\includesvg[width=\linewidth]{alg1_multiple}
   \caption{Algorithm~\ref{alg:vigil} with multiple failures. The drop rates on the links
   are heavily skewed. Prior work have noted the difficulty of detecting links with high drop rates in such scenarios.
   \Sys, however, continues to exhibit high precision/recall.}
		\label{fig:alg1Multiple}
		\vspace{2mm}
\end{figure}




\subsection{Effects of Network size}
\vspace{1mm}

In our final experiment, we explore how \Sys performs as the network
size grows. We observe that its accuracy was on average~$98\%$ when
the network consisted of $1$ pod, $92\%$ for $2$ pods, $91\%$ for $3$
pods, and $90\%$ for $4$ pods when finding a single link failure. In
contrast, the optimization problem~\eqref{opt:integer} had an average
accuracy of~$94\%$, $72\%$, $79\%$, and $77\%$ for the respective
number of pods.


%As the network grows, so does the number of links. For example, in
%the case of $6% pods, out of~$12480$ links in the 6 pod case).

We further evaluate both \Sys and the optimization's ability to find
the cause of per connection drops when the number of failed links in
the network was~$\ge 30$. We observe that both approach's performance
remained unchanged for the most part, e.g., the accuracy of \Sys in
identifying drop causes in an example with $30$ failed links is
$98.01\%$. Figure~\ref{fig:npod} shows the performance (recall) of
using Algorithm~\ref{alg:vigil} as the pod sizes vary. We observe that
recall stayed high even as the network increases in size. The
precision was always $100\%$ and we omit the graph for brevity.


%Finally, the results of using 
%different pod sizes are shown in 

%. 


% where we only
%display its recall because its precision was always~$100\%$.


\begin{figure}[tb]
	\centering
	\includesvg{npod}
	\caption{Recall of Algorithm~\ref{alg:vigil} for different numbers of pods. A six pod network consists of $12480$ links. In all cases
	\Sys continues to have Recall higher than $90\%$. Note, that its precision is $100\%$ for all cases. }
		\label{fig:npod}
\end{figure}

%In this section we only provide
%one example evaluating the accuracy of
%Algorithm~\ref{alg:vigil}. 




%We next investigate its ability to find the links with the highest drop rates, as mentioned in section~\ref{sec:vote} as each connection is likely to go through only one of these failed links at each point in time if \Sys can detect these links reliably it can also detect the cause of packet drops on individual connections (as demonstrated already in Figure~\ref{fig:dropRate}b).





%\noindent{\textbf{Multiple failures when the number of failures is
%    known.}} This investigation allows us to test the hypothesis that
%the $k$ links with the highest scores are indeed the failed links and
%the ordering of the links is representative of the drop rates on the
%links. As shown in~\cite{alex} it is harder to detect failed links in
%the presence of multiple failures especially if there is a large skew
%in the drop rates of these links. Thus, in this experiment, we
%partition the set of failed links such that a random subset (of size
%at least one) has a drop rate chosen uniformly at random between
%$(0.1,1)$ and the rest between $(0.0001,0.01)$. Figure~\ref{fig:multiple} illustrates the results. Again we can see that \Sys performs equally as well when compared to both optimization methods.
%
%
%\begin{figure}[tb]
%	\centering
%	\includesvg{MultipleFailuresWithHighPacketDrops}
%	\caption{Multiple link failures when the number of failed links is known.}
%		\label{fig:multiple}
%\end{figure}




%MultiFailure-NumConChange







==> newmotivation.tex <==
\section{Motivating Example}

We motivate \Sys's design by using a concrete example that we have
experienced within our cloud infrastructure, as a result of
intermittent network problems.  

Although these types of network problems last for only a short period of time, they
could result in dire consequences. To give a concrete example,
Figure~\ref{fig:e17} shows the number of ``sporadic'' VM reboots in
our data center that were classified as network related when triaged
(our definition of sporadic events is one where VMs reboot but no
significant outage has occurred, and no other VM in the same cluster
reboots afterwards). These reboots occur when a VM has write/read
operations which trigger connections to a remote storage
service~\TODO{cite storage paper}. In these instances the storage requests fail
or take too long to complete. This causes the VM to panic and reboot
as it has inconsistent state. VM reboots are disruptive to customer
performance and often an explanation is required as to why they
happened.

Prior work, such as NetPoirot~\cite{Netpoirot}, are only able to
pin-point whether a problem lies in storage, compute, or network. However, in the
event of a network failure, the end goal of an operator is to find the specific link that has caused the problem which is a daunting task given the 
number of links and the lack of efficient/effective monitoring. Moreover, the approach
requires explicit fault injections in order to build up a machine
learning-based classification model. 

On the other hand, \Sys allows us to detect the cause of the VM reboot
problem in real-time. In fact, because \Sys requires only TCP
retransmission counts, the detection requires only seconds, and \Sys
is able to detect network related problems even before VM reboot
occurs, for example, identify the errant switch. This potentially
allow us to proactively fix the problem (e.g. reroute around the
problematic switch) before VM reboot failure occurs.

% as we will show in section \TODO{add
%  section} \Sys allows us to detect network related problems even
%before they resulted in VM reboots. Thus, measures can be taken to
%avoid routing through problematic areas while the problem is
%resolved. Furthermore, we found many of the past triage and RCA's
%\TODO{find out what this is short for} were incorrectly classified, in
%fact we pinpointed the cause of these reboots to a single switch. Our
%results show that a system such as \Sys can be extremely valuable in
%diagnosing such problem.


%Intermittent network problems pose a significant problem for the
%operators of DC networks. 




%\TODO{paper architecture goes here.}






%%these reboots occur when the vm performs a write/read operation which triggers connections to a remote storage service (cite storage paper) 
%%if these connections fail or have high completion times, after a number of retries the VM will have inconsistant state and therefore will panic and reboot.

%%These reboots are disruptive to customer performance, and often an explanation is required as to why they occurred. \Sys allows us to detect the cause of these problems in real time.
%%In fact, as we will show in section X \sys allows us to detect problems minutes before they resulted in a vm reboot, thus measures could be taken to avoid routing through problematic areas of the network. Furthermore, going through X many past triages, we found many were incorrectly classified as non-network related, while a network problem existed. Thus, a system like \sys can be extremely valuable in such circumstances.


==> pathdiscovery-tr.tex <==
\section{The path discovery agent} 
\label{sec:pathdiscovery} 
\vspace{1mm}

The path discovery agent uses traceroute functionality to discover the
path of TCP connections that suffer retransmissions. We first ensure
that the number of traceroutes sent by the agent does not overload our
switches (\S\ref{sec:cpu}).  We then briefly describe the key
engineering issues and how we solve them (\S\ref{sec:eng}).  Our data
centers use IP routing and thus the path discovery agent captures the
L3 path. The architecture of the path discovery agent is shown in
Figure~\ref{fig:overview}.


\subsection{ICMP Rate Limiting}
\label{sec:cpu}
\vspace{1mm}

Generating ICMP packets in response to traceroute consumes switch CPU,
which is a valuable resource in a data center.  In our network, there
is a hard cap of $T_\text{max}=100$ on the number of ICMP messages a switch will send per second. We want to limit the traceroute load on the
switches such that the number of ICMP messages is below $T_\text{max}$. To
do so, we first checked the hop count of all host's TCP connections
during a one hour period in one of our production data centers to see
how many connections might go through a $T_3$ switch. We observed that
$97.9\%$ of these connections had a hop count less than or equal to~$5$ and {\em did not} go through a $T_3$ switch. Given
that our network is a Clos topology and assuming that hosts
under a top of the rack switch~(ToR) communicate with hosts under a
different ToR uniformly at random, we show:

\begin{theorem}\label{theorem1}
\vspace{1mm}

The rate of ICMP~packets generated by any switch
due to a traceroute is below~$T_\text{max}$ if the rate~$C_t$ at which
hosts trigger traceroutes is upper bounded as
%
\begin{align}\label{eq:maxC}
    C_t \leq \frac{
        n_1 n_2 T_{max}
    }{
        H \max\left[ n_2, \frac{n_0^2(\npod-1)}{n_0 \npod-1} \right]
    }
        \text{,}
\end{align}
%
where~$n_0$, $n_1$, and $n_2$ are the numbers of ToR, $T_1$, and~$T_2$
switches respectively and~$H$ is the number of hosts under each ToR.

\end{theorem}

\begin{proof}

See appendix.

\end{proof}

For example, the upper bound of $C_t$ in one of our data centers is
$10$. This means that as long as hosts do not open more than $10$
connections per second, we can {\em guarantee} that the number of
traceroutes generated by \Sys will not go above $T_\text{max}$. We use the hard threshold $C_t$ obtained in the above calculation to limit the number of traceroutes allowed on each host to prevent overwhelming the switches. The agent triggers path discovery no more than once every epoch {\em for a given connection} to further limit the number of traceroutes. We use epochs of $30$~seconds. We will show in \S\ref{sec:vote} that this number is sufficient to ensure high accuracies in detecting links dropping packets in the network.





\subsection{Engineering Challenges}
\label{sec:eng}
\vspace{1mm}

\noindent{\bf Using the correct five-tuple:} Like most modern data centers, our network also makes extensive use of ECMP. All packets of a given flow, defined by the so-called five-tuple, follow the same path~\cite{ECMP}. Thus, the traceroute packets must have the same five-tuple as the TCP connection we are attempting to trace. To ensure this, we must account for the use of load balancers.

TCP connections are initiated in our data center in a manner similar
to that described in~\cite{ananta}. The connection is first
established to a virtual IP (VIP) and the SYN packet (containing the VIP
as destination) goes to a software load balancer (SLB) which
assigns that connection to a physical destination IP (DIP) and a
service port associated with that VIP. The SLB then sends a
configuration message to the virtual switch (vSwitch) in the
hypervisor of the source machine that registers that DIP with that
vSwitch. The destination of all subsequent packets in that connection
have the DIP as their destination and do not go through the SLB. In
order for the path of the traceroute packets to match that of the data
packets, its header should contain the DIP and not the VIP. Thus,
before tracing the path of a connection, the path discovery module
first queries the SLB for the VIP-to-DIP mapping for that connection
and uses the DIP as the destination address for the traceroute
packets. Note that there are cases where the TCP connection
establishment itself may fail due to packet loss. Path discovery is
not triggered for such connections. It is also not triggered when the
query to SLB fails to avoid tracerouting the internet.


\vspace{1mm}
\noindent{\bf Re-routing and packet drops:} We must consider the possibility
that the traceroute itself may fail. For example, this may happen if the link
drop rate is very high.  This actually helps us, since it directly pinpoints the
faulty link. Our analysis engine, described in the next section, is able to use
such partial traceroutes. 

A more insidious possibility is that the routing may change by the time
traceroute starts. We use BGP in our data center network. A lossy link
may cause one or more BGP sessions to fail, triggering rerouting.
Then, the traceroute packets may take a different path than the original
connection. 

The design of \Sys helps avoids this problem. The RTTs in a data center are
typically less than 1 or 2 milliseconds, so the TCP sender retransmits a
dropped packet quickly. The ETW framework notifies the TCP monitoring agent
immediately, which invokes the path monitoring agent. The only additional delay
is the time required to query the SLB to obtain the VIP-to-DIP mapping, which is
typically less than a millisecond. Thus, as long as paths are stable for a few
milliseconds after a packet drop, the traceroute packets will follow the same
path as the TCP connection.

Our network also makes extensive use of link aggregation (LAG)~\cite{linkagg}.
However, unless all the links in the aggregation group fail, the L3 path is not
affected.

\vspace{1mm}
\noindent{\bf{Router aliasing}} We note that the problem of router
aliasing~\cite{aliasing} is easily solved in a data center, as we
know the topology, names, and IP addresses of all routers and interfaces. We
simply map the IP's from traceroutes to the switch names (which we have
from the topology).

To summarize, \Sys's implementation is as follows:
Once the TCP monitoring agent notifies the path discovery agent that a
connection has suffered a retransmission, the path discovery agent checks its
cache of discovered path for that epoch and if need be, queries the SLB for the
DIP.  It then sends 15 appropriately crafted TCP packets with TTL values ranging
from $0-15$. In order to disambiguate the responses, the TTL value is also
encoded in the IP ID field~\cite{ip}. This allows for concurrent
traceroutes to multiple destinations.  The TCP packets deliberately carry a
bad checksum to ensure that they do not interfere with the ongoing connection.


==> proofs.tex <==
%!TEX root = main.tex

\section{Proofs}


%\begin{table*}
%\centering
%\caption{Notation and nomenclature}
%	\label{T:notation}
%\begin{tabular}{cc}
%\hline
%$n_\text{pod}$ & Number of pods \\
%\hline
%$n_0$ & Number of top of the rack~(ToR) switches per pod \\
%\hline
%$n_1$ & Number of tier-1 switches per pod \\
%\hline
%$n_2$ & Number of tier-2 switches \\
%\hline
%Level~1 link & Link between ToR and tier-1 switch \\
%\hline
%Level~2 link & Link between tier-1 and tier-2 switch \\
%\hline
%$\calT_0^s$ & Set of all ToR switches in pod $s$ \\
%\hline
%$\calT_1^s$ & Set of all tier-1 switches in pod $s$ \\
%\hline
%$\calT_0$ & Set of all ToR switches~($\calT_0 = \calT_0^1 \cup \dots \cup \calT_0^{\npod}$) \\
%\hline
%$\calT_1$ & Set of all tier-1 switches~($\calT_1 = \calT_1^1 \cup \dots \cup \calT_1^{\npod}$) \\
%\hline
%$\calT_2$ & Set of all tier-2 switches \\
%\hline
%$k$ & Number of failed links in the network \\
%\hline
%$c_u$ & Upper bound on the number of packets per connection \\
%\hline
%$c_l$ & Lower bound on the number of packets per connection \\
%\hline
%$p_g$ & Probability that a good link drops a packet \\
%\hline
%$p_b$ & Probability that a failed link drops a packet \\
%\hline
%$v_g$ & Probability that a good link receives a vote \\
%\hline
%$v_b$ & Probability that a bad link receives a vote \\
%\hline
%$r_g$ & Probability that a good link causes a retransmission~(drops at least one packet) \\
%\hline
%$r_b$ & Probability that a bad link causes a retransmission~(drops at least one packet) \\
%\hline
%\end{tabular}
%\end{table*}




Consider a Clos topology with $\npod$~pods each with~$n_0$ ToR switches each with $H$~hosts. Links between tier-0 and tier-1 switches are referred to as \emph{level~1 links} and links between tier-1 and tier-2 switches are called \emph{level~2 links}~(see Figure~\ref{F:Clos}). Assume that connection occur uniformly at random between hosts under different ToR switches. Also, assume that link failure and connection routing are independent and that links drop packets independently across links and across packets. To make the derivations clearer, we use calligraphic letter~($\calA$) for sets and boldface~($\bA$) to denote random variables. We also use the notation~$[M] = 1,\dots,M$.

\subsection{Proof of Theorem~1}

\begin{proof}

First, note that since the number of hosts below each ToR switch is the same, we can consider that traceroutes are sent uniformly at random between ToR switches at a rate~$C_t H$. Also, note that routing probabilities are the same for links on the same level, so the traceroute rate depends only on whether the link is on level~1 or level~2. Given ECMP, the traceroute rates on a level~1~($R_1$) and level~2~($R_2$) link is given by
%
\begin{equation*}
	R_{1} = \frac{1}{n_1} C_t H
	\text{ and }
	R_{2} = \frac{n_0}{n_1 n_2}
		\frac{n_0 (\npod - 1)}{(n_0 \npod - 1)} C_t H
		\text{.}
\end{equation*}
%
Since~$n_0$ links are connected to a tier-1 switch and~$n_1$ links are connected to a tier-2, the rate of ICMP packets at any links is bounded by~$T \leq \max\left[ n_0 R_1, n_1 R_2 \right]$.
Taking $\max\left[ n_0 R_1, n_1 R_2 \right] \leq T_\text{max}$ yields~\eqref{eq:maxC} (see~\cite{tr} for more detailed proofs).
%
\end{proof}


% For a $\clos(20,8,10,30)$ with $H = 40$~hosts under each ToR and $T_\text{max} = 100$, $C \leq 9.98$~connections per second.




\vspace{-2mm}
\subsection{Proof of Theorem~2}

We prove a more precise statement of Theorem~\ref{T:vigilWorks}.

\begin{theorem}
	\label{T:vigilWorks2}

In a Clos topology with~$n_0 \geq n_2$ and
$\npod \geq 1 + \max \left[ \frac{n_0}{n_1}, \frac{n_2(n_0 - 1)}{n_0(n_0 - n_2)}, 1 \right]$,
\Sys will rank with probability~$(1 - \epsilon)$ the~$k < \frac{n_2 (n_0 \npod - 1)}{n_0 (\npod - 1)}$ bad links that drop packets with probability~$p_b$ above all good links that drop packets with probability~$p_g$ as long as
%
\begin{equation}\label{E:packetCondition}
	p_g \leq \frac{1 - (1-p_b)^{c_l}}{\alpha c_u}
		\text{,}
\end{equation}
%
where~$c_l$ and~$c_u$ are lower and upper bounds, respectively, on the number of packets per connection, $\epsilon \leq 2 e^{-\calO(N)}$, $N$ is the total number of connections between hosts, and
%
\begin{equation}\label{E:alpha}
	\alpha =
    \frac{
        n_0 (4 n_0 - k) (\npod - 1)
    }{
        n_2 (n_0 \npod - 1) - n_0 (\npod - 1) k
    }
		\text{.}
\end{equation}
%
\end{theorem}


Before proceeding, note that the typical scenario in which~$n_0 \geq 2 n_2$ and~$\frac{n_2(n_0 - 1)}{n_0(n_0 - n_2)} \leq 1$, as in our data center, the condition on the number of pods from Theorem~\ref{T:vigilWorks2} reduces to~$\npod \geq 1 + \frac{n_0}{n_1}$.


\begin{proof}

The proof proceeds as follows. First, we show that if a link has higher probability of receiving a vote, then it receives more votes if a large enough number of connections~($N$) are established. We do so using large deviation theory~\cite{ldp}, so that we can show that the probability that this does not happen decreases exponentially in~$N$.


%%%%%%%%%%%%%%%%% LEMMA 1 %%%%%%%%%%%%%%%%%
\begin{lemma}\label{T:whp}

Let~$v_b$~($v_g$) be the probability of a bad~(good) link receiving a vote. If~$v_b \geq v_g$, \Sys ranks bad links above good links with probability~$1-e^{-\calO(N)}$.

\end{lemma}

With Lemma~\ref{T:whp} in hands, we then need to relate the probabilities of a link receiving a vote~($v_b,v_g$) to the link drop rates~($p_b,p_g$). This will allow us to derive the signal-to-noise ratio condition in~\eqref{E:packetCondition}. Note that the probability of a link receiving a vote is the probability of a flow going through the link \emph{and} that a retransmission occurs~(i.e., some link in the flow's path drops at least one packet).



%%%%%%%%%%%%%%%%% LEMMA 2 %%%%%%%%%%%%%%%%%
\begin{lemma}\label{T:scoringProb}

In a Clos topology with~$n_0 \geq n_2$ and
$\npod \geq 1 + \max \left[ \frac{n_0}{n_1}, \frac{n_2(n_0 - 1)}{n_0(n_0 - n_2)}, 1 \right]$, it holds that for~$k \leq n_0$ bad links
%
\begin{subequations}\label{E:scoringProb}
\begin{align}
	v_b &\geq \frac{r_b}{n_0 n_1 \npod}
		\label{E:badScoringProb}
	\\
	v_g &\leq \frac{1}{n_1 n_2 \npod} \frac{n_0(\npod -1)}{n_0\npod -1}
	\left[
		(4 - \frac{k}{n_0}) r_g + \frac{k}{n_0} r_b
	\right]
		\label{E:goodScoringProb}
\end{align}
\end{subequations}
%
where~$r_b$ and~$r_g$ are the probabilities of a retransmission being due to a bad and a good link, respectively.

\end{lemma}


Before proving these lemmata, let us see how they imply Theorem~\ref{T:vigilWorks2}. From~\eqref{E:scoringProb} in Lemma~\ref{T:scoringProb},
%
\begin{equation}\label{E:retransmissionBound}
	r_b
	\geq
	\underbrace{
		\frac{
			n_0 (4 n_0 - k)(\npod -1)
		}{
			n_2(n_0\npod - 1) - n_0 (\npod -1) k
		}
	}_{\alpha} r_g
	\Rightarrow
	v_b \geq v_g
		\text{,}
\end{equation}
%
for~$k < \frac{n_2 (n_0 \npod-1)}{n_0 (\npod - 1)} < n_0$. Thus, in a Clos topology, if~$r_b \geq \alpha r_g$ for $\alpha$ as in~\eqref{E:alpha}, then~$v_b \geq v_g$. However, \eqref{E:retransmissionBound} gives a relation in terms of probabilities of retransmission~($r_g,r_b$) instead of the packet drop rates~($p_g$,~$p_b$). Nevertheless, note that the probability~$r$ of retransmission during a connection with $c$~packets due to a link that drops packets with probability~$p$ is~$r = 1 - (1-p)^c$. Since~$r$ is monotonically increasing in~$c$, we have~$r_b \geq 1 - (1-p_b)^{c_l}$ and~$r_g \leq 1 - (1-p_g)^{c_u}$. Using the fact~$(1-x)^n \geq 1 - nx$ yields~\eqref{E:packetCondition}.
%
\end{proof}




%%%%%%%%%%%%%%%%% PROOF OF LEMMA 1 %%%%%%%%%%%%%%%%%
\begin{proof}[Proof of Lemma~\ref{T:whp}]

First, note in a datacenter-sized Clos network, almost every connection has a hop count of~$5$~(in our datacenter, this happens to~$97.5\%$ of connections). We can therefore approximate links votes by assuming all bad votes have the same value.

Since links cause retransmissions independently across connections, the number of votes of a bad link is a binomial random variable~$\bB$ with parameters~$N$, the total number of connections, and~$v_b$, the probability of a bad link receiving a bad vote. Similarly, let~$\bG$ be the number of votes on a good link, a binomial random variable with parameters~$N$ and~$v_g$. \Sys will correctly rank bad links if~$\bB \geq \bG$, i.e., if bad links receive more votes than good links. This event contains the event~$\calD = \{\bG \leq (1+\delta) N v_g \cap \bB \geq (1-\delta) N v_b\}$ for $\delta \leq \frac{v_b - v_g}{v_b + v_g}$. Using the union bound~\cite{probBook}, the probability of \Sys correctly identifying bad links obeys
%
\begin{equation}\label{E:pBound}
\begin{aligned}
	\Pr(\bB \geq \bG) &\geq
	1 - \Pr\left[ \bG \geq (1+\delta) N v_g \right]
	\\
	&\hphantom{{}\geq 1}
		{}-	\Pr\left[ \bB \leq (1-\delta) N v_b \right]
		\text{.}
\end{aligned}
\end{equation}
%

To proceed, bound the probabilities in~\eqref{E:pBound} using the large deviation principle~\cite{ldp}, i.e., use the fact that for a binomial random variable~$\bS$ with parameters~$M$ and~$q$ and for~$\delta > 0$ it holds that
%
\begin{subequations}\label{E:LDP}
\begin{align}
	\Pr\left[ \bS \geq (1+\delta) q M \right] &\leq
		e^{-M \DKL((1+\delta) q \| q)}
	\\
	\Pr\left[ \bS \leq (1-\delta) q M \right] &\leq
		e^{-M \DKL((1-\delta) q \| q)}
\end{align}
\end{subequations}
%
where $\DKL(q \| r )$ is the Kullback-Leibler divergence between two Bernoulli distributions with probabilities of success~$q$ and~$r$~\cite{infotheory}. The result in Lemma~\ref{T:whp} is obtained by substituting~\eqref{E:LDP} into~\eqref{E:pBound}.
%
\end{proof}
%%%%%%%%%%%%%%%%% END OF PROOF OF LEMMA 1 %%%%%%%%%%%%%%%%%



\begin{figure}[htb]
	\centering
	\includesvg{clos}
	\caption{Illustration of notation for Clos topology used in the proof of Lemma~\ref{T:scoringProb}}
	\label{F:Clos}
	\vspace{-3mm}
\end{figure}



%%%%%%%%%%%%%%%%% PROOF OF LEMMA 2 %%%%%%%%%%%%%%%%%
\begin{proof}[Proof of Lemma~\ref{T:scoringProb}]

Let~$\calT_0$, $\calT_1$, and~$\calT_2$ denote the set of ToR, tier-1, and tier-2 switches respectively~(Figure~\ref{F:Clos}). Let~$\calT_0^s$ and~$\calT_1^s$, $s = [\npod]$, denote the tier-0 and tier-1 switches in pod~$s$, respectively. Note that~$\calT_0 = \calT_0^1 \cup \dots \cup \calT_0^{\npod}$ and~$\calT_1 = \calT_1^1 \cup \dots \cup \calT_1^{\npod}$. Throughout the derivation, we use subscripts to denote the switch tier and superscripts to denote its pod. For instance, $i_0^s$ is the $i$-th tier-0 switch from pod~$s$, i.e., $i_0^s \in \calT_0^s$, and~$\ell_2$ is the $\ell$-th tier-2 switch~(tier-2 switches do not belong to specific pods). We write~$(i_0^s,j_1^s)$ for the level~1 link between~$i_0^s$ to~$j_1^s$~(as in Figure~\ref{F:Clos}) and~$r(i_0^s,j_1^s) = r(j_1^s,i_0^s)$ to refer to the probability of link~$(i_0^s,j_1^s)$ causing a retransmission.


To get the lower bound in~\eqref{E:badScoringProb}, note that a bad link receives at least as many bad votes as retransmissions it causes. Therefore, the probability of \Sys voting for a bad link is larger than the probability of that link causing a retransmission. The bound is obtained by taking the minimum between the probability of a connection going through a level~1 and a level~2 link and that link causing a retransmission, i.e.,
%
\begin{align*}
	v_b &\geq \min \left[
		\frac{1}{n_0 n_1 \npod},
		\frac{1}{n_1 n_2 \npod} \frac{n_0 (\npod - 1)}{n_0 \npod - 1}
	\right] r_b
		\text{.}
\end{align*}
%
The assumption that~$\npod \geq 1 + \frac{n_2 (n_0 - 1)}{n_0 (n_0 - n_2)}$ makes the first term smaller than the second and yields~\eqref{E:badScoringProb}.


In contrast, the upper bound in~\eqref{E:goodScoringProb} is obtained by applying the union bound~\cite{probBook} over all possible ways that level~1 and level~2 link could be voted. Then, finding an adversarial placement of good and bad links that maximizes the probability of the good link receiving a vote, we find that for~$n_0 \geq n_2$, $\npod \geq 2$, and~$k \leq n_2$, the worst case is achieved for a level~2 link, yielding~\eqref{E:badScoringProb}.
%
\end{proof}
%%%%%%%%%%%%%%%%% END OF PROOF OF LEMMA 2 %%%%%%%%%%%%%%%%%








==> voting-tr.tex <==
\Section{The Analysis Agent}
\label{sec:vote}

Next we describe the analysis agent, focusing first on its voting-based scheme, before presenting an analytical optimal solution that is NP-hard for comparison.



\subsection{Voting Based Scheme}
    \label{sec:votingdetails}
    \vspace{1mm}

\Sys's analysis agent operates based on a simple voting scheme. If a
connection sees a retransmission, \Sys votes the links of that
connection to be \emph{bad}. Each vote carries a value that is tallied at the end of
each epoch, giving a natural ranking of each link in the network. We set the value of good votes
to~$0$ (if a connection has no retransmission, no traceroute
needs to be issued). Bad votes are assigned a value of~$\frac{1}{h}$,
where~$h$ is the number of hops on the path since every link on
the path is equally likely to be responsible for the drop.

The ranking obtained by \Sys after tallying the votes allows us to
identify the most likely cause of packet drops on each connection by
comparing their ranking (which are higher for links with higher drop rates). To further
guard against high levels of noise, we can use our knowledge of the
topology. Namely, when finding the rankings, the votes of the links
lower in the list can be adjusted (assuming ECMP distributes
connections uniformly at random) using an approximation of the number
of votes due to the links higher up in the list. We saw in our evaluations that this can result in a $5\%$ reduction in
the number of false positives.

Note, that \Sys can also be used to find the most problematic links in
the network at each point in time. This can be done using
Algorithm~\ref{alg:vigil}. The algorithm first sorts the links based on their votes. It then checks
whether the top voted link's votes are higher than $1\%$ of the total votes cast. If not, it stops. If yes, it marks it as
one of the most problematic links, removes it from the set of links, and adjusts the votes of the remaining links as described earlier. It continues
to iterate in this manner until the stop criterion is met.

\begin{algorithm}
 \begin{algorithmic}[1]
\STATE $\mathcal{L} \gets$  \text{Set of all links}\\
\STATE $\mathcal{P} \gets$ \text {Set of all {\em possible} path}\\
\STATE $v(l_i) \gets$ \text{Number of votes for $l_i \in \mathcal{L}$}\\
\STATE $\mathcal{B} \gets$ \text{Set of most problematic links}\\
\STATE $l_{max} \gets \text{Link with the maximum votes out of $\forall l_i \in \mathcal{L} \cap \mathcal{B}^c$}$\\
\WHILE{$ v(l_{max}) \ge 0.01(\sum_{l_i \in \mathcal{L}} v(l_i))$}
  \STATE $ l_{max} \gets \max_{l_i \in \mathcal{L} \cap \mathcal{B}^c} v(l_i)$
  \STATE $\mathcal{B} \gets \mathcal{B} \cup \{l_{max}\}$
  \FOR {$l_i \in  \mathcal{L} \cap \mathcal{B}^c$}
  \IF{ $\exists \quad p_i \in \mathcal{P} \quad \text{s.t. } l_i \in p_i  \text{ \& }  l_{max} \in p_i$}
  \STATE Adjust the score of $l_i$
  \ENDIF
  \ENDFOR
\ENDWHILE
\RETURN  $\mathcal{B}$
\end{algorithmic}

\caption{Finding the most problematic links in the network.\label{alg:vigil}}
\end{algorithm}


\subsection{Voting Scheme Analysis}
\vspace{1mm}
\label{sec:reliable}

Can \Sys deliver on its promise of finding the most probable cause of
packet drops on each TCP connection? In \Sys's voting scheme
failed
connections contribute to increases in the tally of both good and bad
links. Moreover, in a large data center such as ours, occasional,
lone, and sporadic packet drops can and \emph{will} happen due to good
links (links that have very low drop rates). These failures are akin to ``noise'' and can cause severe
inaccuracies in any detection system~\cite{gestalt}, \Sys
included. Thus, the answer to this question is not obvious. We show that the likelihood of \Sys making
these errors is small. Taking advantage of the fact that we
know our topology~(Clos network):

\begin{theorem}\label{T:vigilWorks}

For~$\npod \geq \frac{n_0}{n_1} + 1$, \Sys will rank with
probability~$1-2e^{-\calO(N)}$ the $k < \frac{n_2 (n_0 \npod - 1)}{n_0
  (\npod - 1)}$ bad links that drop packets with probability~$p_b$
higher than all good links that drop packets with probability $p_g$ if
%
\begin{equation*}
	p_g \leq \frac{1-(1-p_b)^{c_{l}}}{\alpha c_{u}}
\end{equation*}
%
where $N$ is the total number of connections between hosts, $c_l$ and~$c_u$ are lower and upper bounds, respectively, on the number of packets per
connection, and
%
\begin{equation}\label{eq:alpha}
    \alpha =
    \frac{
        n_0 (4 n_0 - k) (\npod - 1)
    }{
        n_2 (n_0 \npod - 1) - n_0 (\npod - 1) k
    }
        \text{.}
\end{equation}
%

\end{theorem}


\begin{proof}

See appendix.

%\npod \geq 1 + \max \left[ \frac{n_0}{n_1}, \frac{n_2(n_0 - 1)}{n_0(n_0 - n_2)}, 1 \right]

\end{proof}

A single connection is unlikely to go through more
than one ``failed'' link in a network with thousands of links. Theorem~\ref{T:vigilWorks} ensures that the
tally of votes on links with higher drop rates is larger than that of
good links. Combining these two observations allows \Sys to find the
most likely cause of packet drops on each connection.

Note that a straightforward corollary of Theorem~\ref{T:vigilWorks} is
that in the absence of noise~($p_g = 0$), \Sys can pinpoint all bad
links with high probability for large enough~$N$. In the presence of
noise, \Sys can still identify the bad links, as long as the
probability of dropping packets on non-failed links is low
enough~(i.e., the signal-to-noise ratio is large enough). This number,
however, is compatible with typical values found in practice. Indeed,
take as an example~$c_l$ and~$c_u$ to be the $10^{th}$ and $90^{th}$
percentiles, respectively, of the number of packets sent by TCP
connections across all our hosts in a $3$~hour period. If~$p_b \geq 0.5\%$, the packet drop rate on good links can be up to~$1.8 \times 10^{-6}$. For~$p_b \geq 0.05\%$, then Theorem~\ref{T:vigilWorks} only requires~$p_g \leq 7.7 \times 10^{-7}$. Note that packet drop rates in a production data center are typically below~$10^{-8}$~\cite{RAIL}.

Another important consequence of Theorem~\ref{T:vigilWorks} is that it
establishes that the probability of errors in \Sys's results diminishes exponentially
with $N$, so that even with the limits imposed by
Theorem~\ref{eq:maxC} we do not need to use epochs longer
than~$30s$. Moreover, it is worth noting that the conditions in
Theorem~\ref{T:vigilWorks} are sufficient but not necessary. In fact,
\S\ref{sec:sim} illustrates how well \Sys performs even when the
conditions in Theorem~\ref{T:vigilWorks} do not hold~(e.g., for a
larger number of failed links).


 
 

\subsection{Optimal Solution}
\vspace{1mm}
\label{sec:optimal}

While the \Sys's voting scheme works with high probability in a set of situations~(those considered in Section~\ref{sec:reliable}), it is not guaranteed to work in all situations.  In this section, we illustrate an alternative solution in the form of an optimization problem. Given enough resources and time, this method can find the set of links dropping packets on any given connection with high fidelity. The issue is that finding a solution to this optimization problem is NP-hard in general~\cite{bertsimas}. We compare \Sys to this benchmark in our evaluations.


Our goal is to find the most likely cause of failures. This results in
the following optimization problem:
%
\begin{equation}\label{opt:integer}
\begin{aligned}
	\minimize&
	&&\norm{\bm{p}}_0
	\\
	\text{subject to}&
	&&\bm{A} \bm{p} \geq \bm{s}
	\\
	&&&\norm{\bm{p}}_1 = \norm{\bm{s}}_1
	\\
	&&&p_i \in \mathbb{N} \cup \{0\}
\end{aligned}
\end{equation}
%
where $\mathbb{N}$ is the set of natural numbers, $\bm{A}$ is a~$C \times L$ routing matrix, $\bm{s}$ is a~$C \times 1$ vector that collects the number of retransmissions suffered by each connection during an epoch, $L$ is the number of links in the network, $C$ is the number of connections in an epoch, and~$\norm{\bm{y}}_0$ denotes the cardinality of the support of~$\bm{y}$. Note that the $i$-th element of~$\bm{p}$ estimates how many retransmissions were caused by link~$i$, so that it can be used to rank the network links.

The formulation assumes that the minimum subset of links that explain all packet drops is close to representing the set of links dropping packets in reality~(this can be shown to be equivalent to a maximum likelihood formulation). Formulating the problem as~\ref{opt:integer} allows us to relax the stringent~$\bm{A} \bm{p} = \bm{s}$ constraint employed in tomography, which allows for finding the most probable cause of failure. A different binary optimization formulation which only marks the links as good/bad is also possible. In fact, it is the optimization problem that~\cite{netdiagnoser, risk} approximate. Namely,
%
\begin{equation}\label{opt:binary}
\begin{aligned}
	\minimize&
	&&\norm{\bm{p}}_0
	\\
	\text{subject to}&
	&&\bm{A} \bm{p} \geq \bm{s}
	\\
	&&&p_i \in \{0,1\}
\end{aligned}
\end{equation}
%
Similarly to~\eqref{opt:integer}, this minimum set cover formulation is not tractable~(it is NP-complete~\cite{bertsimas}). Moreover, it does not provide a ranking of the links and does not perform well in the presence of noise. Our evaluations showed that \Sys~(Algorithm~\ref{alg:vigil}) significantly outperformed this binary optimization~(by more than $50\%$ in the presence of noise). We illustrate this point in Figures~\ref{fig:reasonable} and~\ref{fig:alg1Single}, but otherwise omit results for this optimization in~\S\ref{sec:sim} for clarity.

In the next three sections, we present our evaluation of \Sys in
simulations~\S\ref{sec:sim}, in a test cluster~\S\ref{sec:test}, and
in one of our production data centers~\S\ref{sec:prod}. 

